Motivations for Early High-Profile FRIB Experiments

This white paper is the result of a collaboration by those that attended a workshop at the Facility for Rare Isotope Beams (FRIB), organized by the FRIB Theory Alliance (FRIB-TA), on Theoretical Justifications and Motivations for Early High-Profile FRIB Experiments. It covers a wide range of topics related to the science that will be explored at FRIB. After a brief introduction, the sections address: (II) Overview of theoretical methods, (III) Experimental capabilities, (IV) Structure, (V) Near-threshold Physics, (VI) Reaction mechanisms, (VII) Nuclear equations of state, (VIII) Nuclear astrophysics, (IX) Fundamental symmetries, and (X) Experimental design and uncertainty quantification.

==> ExpDesign/expdesOLD.tex <==
% * The manuscript is divided up by section, with each section placed in a folder. These folders contain a tex file and any other relevant files (e.g. figures).
% * When adding a block of text, please add a comment at the beginning of the block with your name so that others know who to contact for questions/discussions.
% * All references will be added to a single bibtex file “references.bib”.

%Is up to us to decide what we want to be covered here. Anyone interested in contributing can propose subtopics below.

Given all the areas discussed above, what experiments do we need to run at FRIB? These decisions will be guided by our physics knowledge and biases on what we believe could be impactful, but should be supported on solid statistical grounds. 


We should reference the recent reviews on machine learning, advanced computation, and statistics methods that have been applied to the theory-experiment cycle.
Mention how ``impactful/high-profile" discoveries (or the adjective we decide to use) must also be robust in terms of quantified uncertainties.
%The measurement of the mass of $^{80}$Zr~\cite{hamaker2021precision} could be a good example of an impactful robust discovery, since it is the collective of theoretical mass models under the Bayesian Model Averaging framework that fails to reproduce it (not a single model), signaling a common area for improving our understanding.


\begin{figure*}[!h]
    \centering{\includegraphics[width=0.95\textwidth]{ExpDesign/ExpThCycle.png}}
    \caption{We could use a figure like this (\emph{Adapted from: Colloquium: Machine learning in nuclear physics (2022)})}
      
    \label{fig:Exp_design}
\end{figure*}

% This can go in conclusions
% The reason why: 
% All of these sections are mentioning what theory stands to gain from these experiments. This is a statistics section so I think the outlook stuff is general purpose and should be MORE IMPORTANT and put in general conclusion.

% A lot of these statistical comments should be 'self-evident' and should be seen by everyone ? 

%In conclusion, theory stands to benefit broadly from experimental blah blah, enabled by close collaborative engagement and statistical blah blah

%The "problem" that I see is that this whole section is kind of the main purpose of the whole paper (IS A SELF SIMILAR FRACTAL!), so what I was thinking for a conclusion of this section it is indeed a good part of the conclusion of the whole paper. So I agree, we can lay in this section the reviews and some of the new ideas we have, and then end the conclusion of the paper with these plans and propositions 

% I guess it depends how 'silo-ed' they want the sections :<

%Yep...

\KG{The next part can perhaps go in the main conclusions}

We could end this section with an outlook on how we propose to use these methods, and develop new ones, to make a dynamical motivation/focus for experiments.
Dynamical in the sense that, as we gather new data, the whole theory machinery can swiftly re-calibrate models, quantify how much information was gain in which areas, and continuously re-asses where the most important questions lay next.


Maybe it would be a good idea to suggest that this topical program should be hosted with some regularity (every 2-3 years?) to keep the communication fluid between the theory and experimental fronts.
It would not hurt to invite some of the statisticians/computational collaborators for the next ones, if we decide to go on that route.


\subsection{Raw ideas/topics}

\begin{itemize}
    \item Motivate somewhere the publication of as much data as possible (in raw form) from every experiment that is done to aid in data mining efforts (including the re-adjustment of calculated rates vs observed ones).
    \item We should (definitely!) emphasise the use of pseudo-data analyses to better control the model dependence on our conclusions. For example, if we claim that an experiment X will be a sensitive probe for quantity Y, we should run simulations/calculations with realistic experimental uncertainties structures in the pseudo-data and estimate with which confidence we recover the true Y from the simulated X data.
    \item {\it Xilin:   we can mention that fast emulators for complex bound and continuum state calculations are being developed. They eventually can be fundamental in enabling UQ and experimental design. } 
\end{itemize}



\subsection{Emulators}
In this discovery eigene/cycle, a critical component is the so-called fast emulators for theoretical models/calculations. Many-body calculations of nuclear bound, either in ab initio or DFT frameworks, are computationally expensive. The continuum state calculations face even bigger challenges, since for even few-body systems, the calculations have already become expensive. Therefore, to enable the cycle, the computing costs for these calculations have to be dramatically reduced. The fast emulators offer a solution to this by separating the calculation to two stages: the offline stage (or known as training state in ML) and the online stage (or emulation stage). At the offline stages, the emulators are trained using the high-fidelity solutions of the theoretical models. The computing costs for those high-fidelity solutions should be easily parallelized. At the online stage, the calculations (or rather interpolations and extrapolations in the model input parameter space) need to be fast and accurate. Recently, the nuclear theory community have embraced both data-driven emulations, including Gaussian process, and projection-based emulations (also known as eigenvector continuation) from model reduction field. 

These emulators not only enable efficient exploration of the model input parameter space but also serve as a messenger between the developers of the high-fidelity calculations and other users. For the latter purpose, the emulators are effectively an interface for the users to access the complex models without incurring significant computing costs and without needing the model expertise. As a result, the complex nuclear physics models become more accessible. The closer connections between these models and users will undoubtedly generate novel studies within or even outside the discovery cycle/engine. 


\subsection{A subsection}
